Fine-Tuning and Training of DenseNet for Histopathology Image Representation Using TCGA Diagnostic Slides

Feature vectors provided by pre-trained deep artificial neural networks have become a dominant source for image representation in recent literature. Their contribution to the performance of image analysis can be improved through finetuning. As an ultimate solution, one might even train a deep network from scratch with the domain-relevant images, a highly desirable option which is generally impeded in pathology by lack of labeled images and the computational expense. In this study, we propose a new network, namely KimiaNet, that employs the topology of the DenseNet with four dense blocks, fine-tuned and trained with histopathology images in different configurations. We used more than 240,000 image patches with 1000x1000 pixels acquired at 20x magnification through our proposed "highcellularity mosaic" approach to enable the usage of weak labels of 7,126 whole slide images of formalin-fixed paraffin-embedded human pathology samples publicly available through the The Cancer Genome Atlas (TCGA) repository. We tested KimiaNet using three public datasets, namely TCGA, endometrial cancer images, and colorectal cancer images by evaluating the performance of search and classification when corresponding features of different networks are used for image representation. As well, we designed and trained multiple convolutional batch-normalized ReLU (CBR) networks. The results show that KimiaNet provides superior results compared to the original DenseNet and smaller CBR networks when used as feature extractor to represent histopathology images.

==> Pics/TCGA_Table_Horizon_top3.tex <==

\begin{table}[t]
\centering
\scriptsize
\caption{3-Nearest Neighbors  accuracy (\%) for the horizontal search among 744 WSIs for differently fine-tuned/trained KimiaNet. The best results are highlighted. The last column shows the improvement of accuracy (\%) through KimiaNet compared to DenseNet.}

\begin{tabular}{lc||c||cccc||c}
Tumor Type       & Patient \# & DN                                 & I                                 & II                                 & III                                 & IV                                 & diff  \\ 
\hline
Brain            & 74         & 72 & 96                                 & 97                                 & {\cellcolor[rgb]{0.749,1,0.749}}99 & {\cellcolor[rgb]{0.749,1,0.749}} 99                                 & +27   \\
Breast           & 91         & 53 & 86                                 & 87                                 & {\cellcolor[rgb]{0.749,1,0.749}}91 & {\cellcolor[rgb]{0.749,1,0.749}} 91                                 & +38   \\
Endocrine        & 72         & 65 & 86                                 & 89                                 & {\cellcolor[rgb]{0.749,1,0.749}}93 & 92                                 & +28   \\
Gastro. & 88         & 53                                 & 74                                 & 81                                 & 80                                 & {\cellcolor[rgb]{0.749,1,0.749}}84 & +31   \\
Gynaec.   & 30         & 13 & 43                                 & 40                                 & 47                                 & {\cellcolor[rgb]{0.749,1,0.749}}57 & +44   \\
Head/neck    & 32         & 25 & 75                                 & 69                                 & 81                                 & {\cellcolor[rgb]{0.749,1,0.749}}88 & +63   \\
Liver            & 51         & 43 & 67                                 & 69                                 & 80                                 & {\cellcolor[rgb]{0.749,1,0.749}}88 & +45   \\
Melanocytic      & 28         & 18 & 57                                 & 54                                 & 75                                 & {\cellcolor[rgb]{0.749,1,0.749}}86 & +68   \\
Mesenchymal      & 13         & 23 & 38                                      & 62                                 & {\cellcolor[rgb]{0.749,1,0.749}} 69              &    {\cellcolor[rgb]{0.749,1,0.749}}    69           & +46   \\
Prostate/testis  & 53         & 57 & 89                                 & 91                                 & 94                                 & {\cellcolor[rgb]{0.749,1,0.749}}96 & +39   \\
Pulmonary        & 86         & 56 & 83                                 & {\cellcolor[rgb]{0.749,1,0.749}}86 & 85                                 & {\cellcolor[rgb]{0.749,1,0.749}}86                                 & +30   \\
Urinary tract    & 123        & 59 & {\cellcolor[rgb]{0.749,1,0.749}}89 & {\cellcolor[rgb]{0.749,1,0.749}}89                                 & 88                                 & {\cellcolor[rgb]{0.749,1,0.749}}89                                 & +30  
\end{tabular}
\label{tab:Horizontal}
\end{table} 

%-----------------
\begin{figure}[t]
\centerline{\includegraphics[width=\columnwidth]{Pics/Corrected_Vertical_Search_diag.pdf}}
\caption{Horizontal search results (accuracy, in percentage) for TCGA data.}
\label{fig:Horizontal}
\end{figure}
%----------------------

